Is this Generated Person Existed in Real-world? Fine-grained Detecting and Calibrating Abnormal Human-body

Recent improvements in visual synthesis have significantly enhanced the depiction of generated human photos, which are pivotal due to their wide applicability and demand. Nonetheless, the existing text-to-image or text-to-video models often generate low-quality human photos that might differ considerably from real-world body structures, referred to as "abnormal human bodies". Such abnormalities, typically deemed unacceptable, pose considerable challenges in the detection and repair of them within human photos. These challenges require precise abnormality recognition capabilities, which entail pinpointing both the location and the abnormality type. Intuitively, Visual Language Models (VLMs) that have obtained remarkable performance on various visual tasks are quite suitable for this task. However, their performance on abnormality detection in human photos is quite poor. Hence, it is quite important to highlight this task for the research community. In this paper, we first introduce a simple yet challenging task, i.e., \textbf{F}ine-grained \textbf{H}uman-body \textbf{A}bnormality \textbf{D}etection \textbf{(FHAD)}, and construct two high-quality datasets for evaluation. Then, we propose a meticulous framework, named HumanCalibrator, which identifies and repairs abnormalities in human body structures while preserving the other content. Experiments indicate that our HumanCalibrator achieves high accuracy in abnormality detection and accomplishes an increase in visual comparisons while preserving the other visual content.

==> sec/6_discussion.tex <==
\section{Disscussion}
\label{sec:disscussion}
In this section, we discuss some assumptions and details within our HumanCalibrator.

\textbf{Why do current VLMs lack the ability to perceive abnormality?} It is worth noting that an important assumption of our work is that existing VLMs are unable to perceive detailed human abnormalities, even though this task is very simple for humans, and both we humans and the models are trained on a large amount of normal data. In this work, we conducted numerous experiments to validate this view. Subsequently, our analysis suggests that the drawbacks arise from the simplistic image-text alignment approach of existing VLMs, which lacks perception of content and, consequently, an understanding of human body structure.




\textbf{Does is it necessary to regenerate?} Opting for regeneration using a text-to-video model with similar capabilities rather than a stronger video generation model is mainly for two reasons: (1) The current capabilities of models are still limited, and even the most powerful open-source video models still produce a large number of videos containing anomalies. Using the regeneration approach, it is possible to retain other normal content while also improving the overall quality of the video. (2) The evaluation of human values (abnormal human body structures) can be incorporated into the training process in the future as part of RLHF (Reinforcement Learning from Human Feedback), further enhancing the model's generation performance.
